Learning General Audio Representations with Large-Scale Training of Patchout Audio Transformers

The success of supervised deep learning methods is largely due to their ability to learn relevant features from raw data. Deep Neural Networks (DNNs) trained on large-scale datasets are capable of capturing a diverse set of features, and learning a representation that can generalize onto unseen tasks and datasets that are from the same domain. Hence, these models can be used as powerful feature extractors, in combination with shallower models as classifiers, for smaller tasks and datasets where the amount of training data is insufficient for learning an end-to-end model from scratch. During the past years, Convolutional Neural Networks (CNNs) have largely been the method of choice for audio processing. However, recently attention-based transformer models have demonstrated great potential in supervised settings, outperforming CNNs. In this work, we investigate the use of audio transformers trained on large-scale datasets to learn general-purpose representations. We study how the different setups in these audio transformers affect the quality of their embeddings. We experiment with the models' time resolution, extracted embedding level, and receptive fields in order to see how they affect performance on a variety of tasks and datasets, following the HEAR 2021 NeurIPS challenge evaluation setup. Our results show that representations extracted by audio transformers outperform CNN representations. Furthermore, we will show that transformers trained on Audioset can be extremely effective representation extractors for a wide range of downstream tasks.

==> removed.tex <==

%  added these to clarify the observation of the figure case some of them are difficult to understand from the figure itself , (can be removed)
\subsection{score table for low level features}

\begin{table}[h!]
\centering
\caption{Comparison of PaSST models with different embedding levels}
\label{table:dm_base}
\begin{tabular}{ |m{12em}| c| c| }
 \hline
 \textbf{Model} &  \textbf{DCASE} & \textbf{MAESTRO} \\
 \hline
 Cat xwc   &   0.680804   &   0.469077\\
 PaSST+L+M   &   0.850361   &   0.432946\\
 PaSST+L+M+H   &   0.832132   &   0.327444\\
 PaSST+M   &   0.796646   &   0.039797\\
 Wav2vec2   &   0.662996   &   0.032896\\
 PaSST+M+H   &   0.809573   &   0.024657\\
 PaSST+H   &   0.772936   &   0.021537\\
 OpenL3   &   0.832780  &    0.016502\\
 \hline

\end{tabular}
\end{table}



\subsection{score table receptive field}

\begin{table}[h!]
\centering
\caption{Comparison of PaSST L+M models with different RFs}
\label{table:dm_rf}
\begin{tabular}{ |m{14em}| c| c| }
 \hline
 \textbf{Model} &  \textbf{DCASE} & \textbf{MAESTRO} \\
 \hline
 Cat xwc   &   0.680804   &   0.469077\\
 PaSST+L+M   &   0.850361   &   0.432946\\
 PaSST+L+M+2RF    &  0.916402  &    0.426333\\
 PaSST+L+M High RF   &   0.931477    &  0.419773\\
 Wav2vec2    &  0.662996   &   0.032896\\
 OpenL3   &  0.832780   &   0.016502\\
 \hline
\end{tabular}
\end{table}

% remove the subsection completely ?
\subsection{different RF}
% @shahed, 
% 1) different window sizes: (careful about the limits)

\begin{figure}[h!]
\centering
{\includegraphics[width=1.0\textwidth]{figs/results/DM_win.png}}
\caption{compare L+M+2RF models with \textit{hop=10 ms} different larger 2RF size}
\label{fig:dm_win}
\end{figure}

\begin{table}[h!]
\centering
\caption{Comparison of PaSST L+M+2RF models and different larger 2RF size}
\label{table:dm_win}
\begin{tabular}{ |m{14em}| c| c| }
 \hline
 \textbf{Model} &  \textbf{DCASE} & \textbf{MAESTRO} \\
 \hline
 PaSST+L+M+2RF    &  0.916402   &   0.426333\\
 PaSST+L+M+2RF win=180   &   0.934322  &    0.407076\\
 PaSST+L+M+2RF win=200   &   0.943194    &  0.401626\\
 \hline
\end{tabular}
\end{table}

